On Transferability of Bias Mitigation Effects in Language Model Fine-Tuning

Fine-tuned language models have been shown to exhibit biases against protected groups in a host of modeling tasks such as text classification and coreference resolution. Previous works focus on detecting these biases, reducing bias in data representations, and using auxiliary training objectives to mitigate bias during fine-tuning. Although these techniques achieve bias reduction for the task and domain at hand, the effects of bias mitigation may not directly transfer to new tasks, requiring additional data collection and customized annotation of sensitive attributes, and re-evaluation of appropriate fairness metrics. We explore the feasibility and benefits of upstream bias mitigation (UBM) for reducing bias on downstream tasks, by first applying bias mitigation to an upstream model through fine-tuning and subsequently using it for downstream fine-tuning. We find, in extensive experiments across hate speech detection, toxicity detection, occupation prediction, and coreference resolution tasks over various bias factors, that the effects of UBM are indeed transferable to new downstream tasks or domains via fine-tuning, creating less biased downstream models than directly fine-tuning on the downstream task or transferring from a vanilla upstream model. Though challenges remain, we show that UBM promises more efficient and accessible bias mitigation in LM fine-tuning.

==> chaps/discards.tex <==
 %Here we consider the case of fine-tuning models to classification tasks. %\xiang{why not narrow down to PTLMs in this section? given this is what the Intro narrative and your exps focus on.}
%Specifically, we consider a transfer learning scenario in which fine-tuning is initially performed on source domains and tasks (i.e., \textit{upstream} fine-tuning), and the fine-tuned encoder is transferred to a target domain and task for \textit{downstream} fine-tuning. 

%Fine-tuning on (pre-)trained weights has become a common and effective practice in natural language processing. A significant advantage of fine-tuning is its simplicity: model developers simply load (pre-)trained weights and transfer the strong inductive bias implicitly stored in the weights to the target task by fine-tuning.

%Formally, we suppose a model $f = g \circ h$ is composed by a text encoder $g$ (\eg, Transformers) that output a sentence representation $\rvh\in \R^n$, and a classifier head $h$, typically a linear layer, that takes the representation $\rvh$ as input and output a label $y$. In the transfer learning setup, a model $f_s = g \circ h_s$ is trained on a source domain $\mathcal{D}_s$. Then, only the text encoder $g$ is passed to the target domain $\mathcal{D}_t$ to compose a new model $f_t = g \circ h_t$, where $h_t$ is freshly initialized. Both the encoder $g$ and the new classifier head $h_t$ are trained jointly in the target domain.

%Fine-tuning a PTLM consists of a pretrained encoder fine-tuned to a particular task for a downstream dataset. 
%Formally, fine-tuning requires a neural classification model $f: \R^m \to \{0,1,...,C\}$, which maps an input sentence $\rvx$ to a class label $y$. The model $f=h \circ g$ is composed of a \textit{text encoder} $g: \R^m \to \R^d$ (\eg, Transformers in RoBERTa~\citep{Liu2019RoBERTaAR}) which maps an input sentence $\rvx$ to a hidden representation $\rvz \in \R^d$ in the representation space; and a \textit{classifier head} $h: \R^d \to  \{0,1,...,C\}$, which maps the representation $\rvz$ to the label space. The model is trained on a dataset of examples $(\rvx, y)$ from a domain $\mathcal{D}$ for a task $\mathcal{T}$: the domain describes the input space $\mathcal{X}$ and its marginal distribution, and the task $\mathcal{T}$ describes the label space $\mathcal{Y}$ and the predictive function to learn. 
%To adapt a classification model from a source domain $\mathcal{D}_s$ (trained for a source task $\mathcal{T}_s$) to a target domain $\mathcal{D}_t$ (for a target task $\mathcal{T}_t$), one first trains
%the model $f_s=h_s \circ g_s$ in the source data $(\rvx^s, y^s)$, yielding the source (upstream) model. Then, for transfer learning to $\mathcal{D}_t$ and implementing the downstream (target) model $f_t = h_t \circ g_t$ for task $\mathcal{T}_t$, the upstream encoder $g_s$ is used to initialize the weights of downstream encoder $g_t$, while the classifier head $h_t$ is randomly initialized. The full target model $f_t$ is then trained on the target data $(\rvx^t, y^t)$. Note that the upstream model itself can also be obtained via fine-tuning from an upper-stream model, for example, PTLMs, which is the practice we apply.
%\textbf{Upstream and Downstream Finetuning.} In our proposed transfer learning framework, we consider multiple instances of fine-tuning for a given PTLM, occurring on potentially different domains. We use the notion of ``upstream'' and ``downstream'' to refer to the prior and latter fine-tunings of the same model. Formally, a classification model can be adapted from a source domain $\mathcal{D}_s$ trained for a source task $\mathcal{T}_s$ to a target domain $\mathcal{D}_t$ for a target task $\mathcal{T}_t$. One first trains the model $f_s=h_s\circ g_s$ in source domain $\mathcal{D}_s$, yielding the source (upstream) model. Then, for transfer learning to $\mathcal{D}_t$ and implementing the downstream (target) model $f_t = h_t \circ g_t$, the upstream encoder $g_s$ is used to initialize the weights of downstream encoder $g_t$ and the classifier head $h_t$ is randomly initialized. The full target model $f_t$ is then trained on the target domain $\mathcal{D}_t$ for the target task $\mathcal{T}_t$.
%\xiang{reads more like belonging to proposed work part, because mixing with some of our framework ideas. Clean it up a bit and only touch on previous work and its issue.}

%\textbf{Fine-tuning.} In our proposed transfer learning framework, we consider multiple instances of fine-tuning for a given PTLM, occurring on potentially different domains. We use the notion of ``upstream'' and ``downstream'' to refer to the prior and latter fine-tunings of the same model. Formally, a classification model can be adapted from a source domain $\mathcal{D}_s$ trained for a source task $\mathcal{T}_s$ to a target domain $\mathcal{D}_t$ for a target task $\mathcal{T}_t$. One first trains the model $f_s=h_s\circ g_s$ in source domain $\mathcal{D}_s$, yielding the source (upstream) model. Then, for transfer learning to $\mathcal{D}_t$ and implementing the downstream (target) model $f_t = h_t \circ g_t$, the upstream encoder $g_s$ is used to initialize the weights of downstream encoder $g_t$ and the classifier head $h_t$ is randomly initialized. The full target model $f_t$ is then trained on the target domain $\mathcal{D}_t$ for the target task $\mathcal{T}_t$.







%When dealing with multiple bias factors, the upstream model $f_s$ may be jointly trained on several datasets with domains $\mathcal{D}_s^{1:K}$ for tasks $\mathcal{T}_s^{1:K}$ (noted as domain-task pairs $\langle\mathcal{D}_s, \mathcal{T}_s \rangle^{1:K}$). We assume each source domain-task pair $\langle \mathcal{D}_s^j, \mathcal{T}_s^j \rangle$ is dedicated to address a single bias factor $a^{(j)}$, sharing the same superscription. 
%The joint training can be formulated as a multi-task learning problem, where the encoder $g_t$ is shared and the classifier head $h_t^{j}$ is specific to each domain-task pair. Specifically, we consider two dimensions of settings, specifying: (1) the similarity between the source and the target domain and the task, and (2) the number of bias factors considered. Settings can vary based on these two dimensions (Figure~\ref{fig:framework} (left)):




\begin{comment}
In the first stage, we train a de-biased classifier with either explanation regularization or adversarial de-biasing in the source domain. The text encoder $g_s$ is then extracted from the full model $f_s = h_s \circ g_s$ and transferred to the target domain for fine-tuning in the second stage. %We expect the encoder $g$ of the de-biased model encodes information about de-biasing and could benefit downstream classifiers.

%\subsection{Model Fine-tuning Algorithms}
%\label{sec:finetune}
%\vspace{-0.2cm}
%\xiang{Have a guiding formulation here will be good.}

Next, in the downstream fine-tuning stage, we train a downstream classifier $f_t = h_t \circ g_t$ in the target domain $\mathcal{D}_t$ for the target task $\mathcal{T}_t$, where $g_t$ is initialized with $g_s$, transferred from the source model. While no de-biasing algorithms are applied in this stage, the model is trained by jointly fine-tuning $g_t$ and $h_t$; in our main experiments, we employ this simple fine-tuning strategy to obtain the target model $f_t$. We also consider two approaches aiming at preserving the de-biased encoder for analysis: (1) the encoder $g_t$ is frozen while only $h_t$ is trained, and (2) the encoder $g_t$ is penalized for deviating from $g_s$ with a regularization term. In the second approach, we use $\ell^2$-sp regularizer~\citep{Li2018ExplicitIB}, which penalizes the distance between the weights and the initial point of fine-tuning. Formally, let $\rvw_0$ be the initial weight of the encoder $g_t$ before fine-tuning, and $\rvw$ be the current weight of $g_t$. The $\ell^2$-sp regularizer is written as $\Omega(\rvw) = \beta || \rvw - \rvw_0 ||^2_2$, where $\beta$ is a hyperparameter controlling the strength of the regularization, set to 1 by default.
\end{comment}
%In the second phase, model developers build a fresh classification head $h_t$ for their own downstream task $g$ upon the encoder and fine-tune the whole model $f_t = h \circ g_t$. %We study two realistic settings, where model developers are either \textit{unconscious} or \textit{conscious} of model de-biasing.

%When model developers are unconscious about model de-biasing, the models are solely fine-tuned for the performance; when model developers are actively trying to reduce bias, they can apply regularization at fine-tuning to retain knowledge about de-biasing encoded in the model.  When $\beta \to \infty$, the regularization is equivalent to freezing the weight of the encoder.




\begin{comment}
% \textbf{Definition of Prediction Bias.}
%Before discussing prediction bias in the context of fine-tuning PTLMs, we first define what we mean by ``\textit{prediction bias}'', and how we measure it based on a model's behaviors. 
The general objective of this paper is to test whether the effects of bias mitigation algorithms transfer in the fine-tuning paradigm. To evaluate models' prediction bias, we operationalize \textit{equal opportunities}~\citep{Hardt2016EqualityOO}: a model $f$ is biased if it yields higher prediction error rates for a certain label over a subset $S$ of the data. In cases where the subset $S$ is associated with a specific social group, lack of \textit{equal opportunities} leads to unfair, biased predictions. %, partitioned by the demographic attributes of authors or explicit mentions of group identifiers in the text. 
We evaluate equal opportunities for various subsets of the data, each associated with a \textit{bias factor}. We refer to each bias factor $a^{(j)}$ with its index $j \in \{0,1,...,K\}$: for example, the subset $S^{(j)}$ may consist of all examples produced by African American English speakers, or all input examples that mention a certain group identifier (\eg, female pronouns). For each sample $(\rvx_i,y_i)$ in the dataset, we use a binary attribute vector $\rva_i \in \{0,1\}^K$ to indicate its associated subsets, where the $j$-th item $a_i^{(j)} \in \{0,1\}$ indicates whether $\rvx_i$ belongs to the set $S^{(j)}$. 

In this paper, we assess equal opportunities regarding \textit{false positive error rates}, given that positives in our label sets (e.g., spam, offensive, hate speech labels) are considered harmful and an incorrect positive prediction leads to some cost for the instance (e.g., offensive posts can get blocked in a social media platform); however, the framework can effortlessly be applied to other cases, \eg, where false negative rates are also considered as the evidence of bias. For simplicity of notations, we use label $y=1$ to refer to harmful outcomes (\eg, spam, or hate speech), and $y=0$ for others. The prediction bias regarding subset $S^{(j)}$ is formally defined as the false positive rate difference (FPRD$^{(j)}$), and is quantified as:
\begin{equation}
\label{eq:fprd}
    \begin{split}
    \textrm{FPRD}^{(j)} = P(\hat{y}=1 | a^{(j)} = 1, y=0) - \\ P(\hat{y}=1 | a^{(j)}=0, y=0),
    \end{split}
\end{equation}
where $\hat{y}$ is the model prediction for a sample. The term $P(\hat{y}=1 |y=0, a^{(j)})$ indicates the false positive rate for bias factor $j$ (FPR$^{(j)}$). In other words FPR$^{(j)}$ shows the probability of predicting a label as positive when the ground truth is negative, conditioned on the value of the attribute $a^{(j)}$. 
\end{comment}

%The explanation regularization approach can be applied when the model is overly sensitive to a particular lexicon, associated with the bias factors. For instance, the model may spuriously associate hate speech labels with data that mentions group identifiers, or language that is commonly used by a certain demographic group, resulting in higher FPRDs. The adversarial de-biasing approach is more general and does not require a predefined set of lexicons.
\begin{comment}


\textbf{Explanation Regularization.} For a source domain and task in $\langle \mathcal{D}_s,\mathcal{T}_s \rangle^{1:K}$ with training examples $(\rvx^s, y^s, \rva^s)$, explanation regularization approaches assign an importance score $\phi^{(j)}(w, \rvx^s)$ for each word $w$ in a predefined lexicon set $\mathcal{W}^{(j)}$ that is present in the input example $\rvx^s$ and indicates an attribute $a^{(j)} \in \rva^s$. When training the upstream model $f_s$ on a set of bias factors, the importance scores are regularized jointly with the main learning objective,
%\begin{equation}
%\label{eq:expl_reg}
%    \min_{f_s} \quad \ell_{c} + \alpha \ \sum^{K}_{j=1} \sum_{w \in \rvx^s \cap \mathcal{W}^{(j)} } %||\phi^{(j)}(w, \rvx^s)||^2
%\end{equation}
where $\ell_{c}$ is the classification loss and $\alpha ||\phi^{(j)}(w, \rvx^s)||^2$ penalizes the importance attributed cumulatively to all $w\in \mathcal{W}^{(j)}$. $\alpha$ is a hyperparameter controlling the strength of the regularization. While a variety of explanation algorithms can be applied to measure $\phi^{(j)}(w, \rvx^s)$, we focus on the simplest input occlusion algorithm~\citep{Zintgraf2017VisualizingDN}, where the importance is quantified as the change in model prediction caused by removing $w$ from the input $\rvx^s$. 

\textbf{Adversarial De-biasing.} For a source domain and task in $\langle \mathcal{D}_s,\mathcal{T}_s \rangle^{1:K}$ with training examples $(\rvx^s, y^s, \rva^s)$, adversarial de-biasing algorithms reduce the predictability of the attributes $\rva^s$ from the intermediate data representations generated by encoder $g_s$. During training, an adversarial classifier head $h_{adv}^{(j)}: \R^{d} \to [0,1]$ is built upon the encoder $g_s$ for each attribute $a^{(j)} \in \rva^s$. The adversarial classifier is trained to predict the attribute $a^{(j)}$ by optimizing the cross entropy loss $\ell_{adv}(h^{(j)}_{adv} \circ g_s(\rvx^s), a^{(j)})$. A gradient reversal layer~\citep{ganin2016domain} is added between the encoder $g_s$ and $h^{(j)}_{adv}$, so that the encoder $g_s$ is optimized to generate representations that do not encode information about the attribute $a^{(j)}$. The adversarial learning objective is optimized jointly with the classification objective at training. Formally, the optimization problem is written as,
\begin{align}
    \min_{g_s,h} \max_{h^{1:K}_{adv}} \quad \ell_c + \sum_{j=1}^{K} \ell_{adv}(h^{(j)}_{adv}  \circ g_s(\rvx^s), a^{(j)})
\end{align}
while the adversarial loss $\ell_{adv}$ can take other forms as in~\cite{Madras2018LearningAF}, we did not observe meaningful differences empirically.
\end{comment}

\begin{comment}
In the first stage, we train a de-biased classifier with either explanation regularization or adversarial de-biasing in the source domain. The text encoder $g_s$ is then extracted from the full model $f_s = h_s \circ g_s$ and transferred to the target domain for fine-tuning in the second stage. %We expect the encoder $g$ of the de-biased model encodes information about de-biasing and could benefit downstream classifiers.

%\subsection{Model Fine-tuning Algorithms}
%\label{sec:finetune}
%\vspace{-0.2cm}
%\xiang{Have a guiding formulation here will be good.}

Next, in the downstream fine-tuning stage, we train a downstream classifier $f_t = h_t \circ g_t$ in the target domain $\mathcal{D}_t$ for the target task $\mathcal{T}_t$, where $g_t$ is initialized with $g_s$, transferred from the source model. While no de-biasing algorithms are applied in this stage, the model is trained by jointly fine-tuning $g_t$ and $h_t$; in our main experiments, we employ this simple fine-tuning strategy to obtain the target model $f_t$. We also consider two approaches aiming at preserving the de-biased encoder for analysis: (1) the encoder $g_t$ is frozen while only $h_t$ is trained, and (2) the encoder $g_t$ is penalized for deviating from $g_s$ with a regularization term. In the second approach, we use $\ell^2$-sp regularizer~\citep{Li2018ExplicitIB}, which penalizes the distance between the weights and the initial point of fine-tuning. Formally, let $\rvw_0$ be the initial weight of the encoder $g_t$ before fine-tuning, and $\rvw$ be the current weight of $g_t$. The $\ell^2$-sp regularizer is written as $\Omega(\rvw) = \beta || \rvw - \rvw_0 ||^2_2$, where $\beta$ is a hyperparameter controlling the strength of the regularization, set to 1 by default.
\end{comment}
%In the second phase, model developers build a fresh classification head $h_t$ for their own downstream task $g$ upon the encoder and fine-tune the whole model $f_t = h \circ g_t$. %We study two realistic settings, where model developers are either \textit{unconscious} or \textit{conscious} of model de-biasing.

%When model developers are unconscious about model de-biasing, the models are solely fine-tuned for the performance; when model developers are actively trying to reduce bias, they can apply regularization at fine-tuning to retain knowledge about de-biasing encoded in the model.  When $\beta \to \infty$, the regularization is equivalent to freezing the weight of the encoder.

==> floats/legacy/par_tabs_dwmw_fdcl.tex <==
\begin{table}
\centering
\vspace{-0.3cm}
\begin{minipage}[t]{0.48\textwidth}
    \centering
    \
    \scalebox{0.64}{\begin{tabular}{@{}l|ccc@{}}
\toprule
\textbf{Method / Datasets}      & \multicolumn{2}{c}{\textbf{DWMW}}                                                                                                                                                                                                              \\ \midrule
\textbf{Metrics}                & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ Acc. ($\uparrow$)\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}BROD\\ Acc. ($\uparrow$)\end{tabular}} \\ \midrule
                                & \multicolumn{2}{c}{\textit{Single dataset}}                                                                                                                                                                                                      \\ \midrule
\textbf{Vanilla}                & \textbf{91.46 $\pm$ 0.1}                                                                                                                               & \textbf{78.77 $\pm$ 0.3}                                                                     \\
\textbf{Expl. Reg.}             & 91.38 $\pm$ 0.1                                                                                                                                        & 76.61 $\pm$ 1.5                                                                     \\
\textbf{Adv. Learning}          & 91.11 $\pm$ 0.3                                                                                                                                    & 77.53 $\pm$ 0.9                                                                     \\ \midrule
\textbf{}                       & \multicolumn{2}{c}{\textit{FDCL $\to$ DWMW}}                                                                                                                                                                                                 \\ \midrule
\textbf{Van-Transfer}          & 91.27 $\pm$ 0.2                                                                                                                                        & 78.98 $\pm$ 1.1                                                                     \\
\textbf{\method$_{Reg}$}    & 91.39 $\pm$ 0.0                                                                                                                                            & \textbf{80.27 $\pm$ 0.2}                                                                     \\
\textbf{\method$_{Adv}$}          & \textbf{91.60 $\pm$ 0.1}                                                                                                                                      & 79.98 $\pm$ 1.7                                                                     \\ \midrule
\textbf{}                       & \multicolumn{2}{c}{\textit{GHC + FDCL $\to$ DWMW}}                                                                                                                                                                                           \\ \midrule
\textbf{Van-Transfer}            & 91.65 $\pm$ 0.1                                                                                                                                      & 80.98 $\pm$ 0.4                                                                     \\
\textbf{\method$_{Reg + Reg}$} & \textbf{91.79 $\pm$ 0.4}                                                                                                                                  & \textbf{81.36 $\pm$ 0.8}                                                                    \\
\textbf{\method$_{Reg + Adv}$}       & 91.33 $\pm$ 0.1                                                                                                                                  & 81.09 $\pm$ 0.4                                                                     \\ \midrule
                                & \multicolumn{2}{c}{\textit{Stf. + FDCL $\to$ DWMW}}                                                                                                                                                                                          \\ \midrule
\textbf{Van-Transfer}            & 91.64 $\pm$ 0.2                                                                                                                                      & 81.12 $\pm$ 0.1                                                                     \\
\textbf{\method$_{Reg + Reg}$} & \textbf{91.66 $\pm$ 0.2}                                                                                                                                          & 80.05 $\pm$ 0.1                                                                     \\
\textbf{\method$_{Reg + Adv}$}       & 91.55 $\pm$ 0.2                                                                                                                                         & \textbf{81.14 $\pm$ 1.5}                                                                     \\ \bottomrule
\end{tabular}}
\vspace{0.1cm}
    \caption{\textbf{Cross-domain and task} transfer with DWMW as the target domain.}
    \label{tab:dwmw_cross_domain}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}[t]{0.48\textwidth}
\centering
\scalebox{0.64}{\begin{tabular}{@{}l|ccc@{}}
\toprule
\textbf{Method / Datasets}      & \multicolumn{2}{c}{\textbf{FDCL (Half-)B}}                                                                                                                                                                                                     \\ \midrule
\textbf{Metrics}                & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ Acc. ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}BROD\\ Acc. ($\uparrow$)\end{tabular}} \\ \midrule
                                & \multicolumn{2}{c}{\textit{Single dataset}}                                                                                                                                                                                                      \\ \midrule
\textbf{Vanilla}                & 75.72 $\pm$ 0.2                                                                                                                          & 73.57 $\pm$ 1.2                                                                     \\
\textbf{Expl. Reg.}             & \textbf{77.30 $\pm$ 0.2}                                                                                                                                     & 76.72 $\pm$ 1.1                                                                     \\
\textbf{Adv. Learning}          & 75.28 $\pm$ 0.2                                                                                                                                         & \textbf{77.12 $\pm$ 1.2}                                                                     \\ \midrule
\textbf{}                       & \multicolumn{2}{c}{\textit{FDCL A $\to$ FDCL B}}                                                                                                                                                                                                 \\ \midrule
\textbf{Van-Transfer}          & \textbf{76.33 $\pm$ 0.6}                                                                                                                            & 70.35 $\pm$ 2.4                                                                     \\
\textbf{\method$_{Reg}$}    & 76.22 $\pm$ 0.5                                                                                                                                       & 69.29 $\pm$ 1.8                                                                     \\
\textbf{\method$_{Adv}$}          & 75.88 $\pm$ 0.4                                                                                                                                      & \textbf{71.11 $\pm$ 1.6}                                                                     \\ \midrule
\textbf{}                       & \multicolumn{2}{c}{\textit{GHC A + FDCL A $\to$ FDCL B}}                                                                                                                                                                                         \\ \midrule
\textbf{Van-Transfer}            & \textbf{77.34 $\pm$ 0.4}                                                                                                                                      & 72.96 $\pm$ 1.5                                                                     \\
\textbf{\method$_{Reg + Reg}$} & 76.21 $\pm$ 0.4                                                                                                                                      & 73.10 $\pm$ 1.4                                                                     \\
\textbf{\method$_{Reg + Adv}$}       & 76.94 $\pm$ 0.4                                                                                                                              & \textbf{76.55 $\pm$ 0.7}                                                                     \\ \midrule
                                & \multicolumn{2}{c}{\textit{Stf. A + FDCL A $\to$ FDCL B}}                                                                                                                                                                                        \\ \midrule
\textbf{Van-Transfer}            & \textbf{77.18 $\pm$ 0.5}                                                                                                                                         & 71.12 $\pm$ 1.2                                                                     \\
\textbf{\method$_{Reg + Reg}$} & 77.13 $\pm$ 0.3                                                                                                                                   & 72.17 $\pm$ 1.6                                                                     \\
\textbf{\method$_{Reg + Adv}$}       & 76.64 $\pm$ 0.6                                                                                                                                  & \textbf{76.55 $\pm$ 0.6}                                                                     \\ \bottomrule
\end{tabular}}
\vspace{0.1cm}
\caption{\textbf{Same-domain and task} transfer with the second half of FDCL as the target domain.}
\label{tab:fdcl_same_domain}
\end{minipage}
\vspace{-0.4cm}
\end{table}

==> floats/legacy/tab_dwmw_cross_domain.tex <==
% Please add the following required packages to your document preamble $\pm$ 
% \usepackage{booktabs}
\begin{table}[]
\centering
\scalebox{0.7}{\begin{tabular}{@{}l|ccc@{}}
\toprule
\textbf{Method / Datasets}      & \multicolumn{3}{c}{\textbf{DWMW17}}                                                                                                                                                                                                              \\ \midrule
\textbf{Metrics}                & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ Acc. ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}BROD16\\ FPRD ($\downarrow$)\end{tabular}} \\ \midrule
                                & \multicolumn{3}{c}{\textit{Single dataset}}                                                                                                                                                                                                      \\ \midrule
\textbf{Vanilla}                & 91.46 $\pm$ 0.1                                                                      & 8.66 $\pm$ 1.0                                                                         & 79.77 $\pm$ 0.3                                                                     \\
\textbf{Expl. Reg.}             & 91.38 $\pm$ 0.1                                                                      & 5.93 $\pm$ 0.2                                                                         & 76.61 $\pm$ 1.5                                                                     \\
\textbf{Adv. Learning}          & 91.11 $\pm$ 0.3                                                                      & 11.60 $\pm$ 0.1                                                                        & 77.53 $\pm$ 0.9                                                                     \\ \midrule
\textbf{}                       & \multicolumn{3}{c}{\textit{FDCL18 $\to$ DWMW17}}                                                                                                                                                                                                 \\ \midrule
\textbf{Van. Transfer}          & 91.27 $\pm$ 0.2                                                                      & 5.59 $\pm$ 1.1                                                                         & 78.98 $\pm$ 1.1                                                                     \\
\textbf{Expl. Reg. Transfer}    & 91.39 $\pm$ 0.0                                                                      & 5.06 $\pm$ 0.8                                                                         & 80.27 $\pm$ 0.2                                                                     \\
\textbf{Adv. Transfer}          & 91.60 $\pm$ 0.1                                                                      & 7.20 $\pm$ 1.0                                                                         & 79.98 $\pm$ 1.7                                                                     \\ \midrule
\textbf{}                       & \multicolumn{3}{c}{\textit{GHC + FDCL18 $\to$ DWMW17}}                                                                                                                                                                                           \\ \midrule
\textbf{Van. + Van.}            & 91.65 $\pm$ 0.1                                                                      & 8.02 $\pm$ 1.1                                                                         & 80.98 $\pm$ 0.4                                                                     \\
\textbf{Expl. Reg + Expl. Reg.} & 91.79 $\pm$ 0.4                                                                      & 8.41 $\pm$ 0.5                                                                         & 81.36 $\pm$ 0.8                                                                     \\
\textbf{Expl. Reg + Adv.}       & 91.33 $\pm$ 0.1                                                                      & 8.75 $\pm$ 1.7                                                                         & 81.09 $\pm$ 0.4                                                                     \\ \midrule
                                & \multicolumn{3}{c}{\textit{Stf. + FDCL18 $\to$ DWMW17}}                                                                                                                                                                                          \\ \midrule
\textbf{Van. + Van.}            & 91.64 $\pm$ 0.2                                                                      & 6.91 $\pm$ 1.0                                                                         & 81.12 $\pm$ 0.1                                                                     \\
\textbf{Expl. Reg + Expl. Reg.} & 91.66 $\pm$ 0.2                                                                      & 6.32 $\pm$ 0.4                                                                         & 80.05 $\pm$ 0.1                                                                     \\
\textbf{Expl. Reg + Adv.}       & 91.55 $\pm$ 0.2                                                                      & 7.83 $\pm$ 1.2                                                                         & 81.14 $\pm$ 1.5                                                                     \\ \bottomrule
\end{tabular}}
\caption{}


\end{table}

==> floats/legacy/tab_fdcl_same_domain.tex <==
% Please add the following required packages to your document preamble $\pm$ 
% \usepackage{booktabs}
\begin{table}[]
\centering
\scalebox{0.70}{\begin{tabular}{@{}l|ccc@{}}
\toprule
\textbf{Method / Datasets}      & \multicolumn{3}{c}{\textbf{FDCL18 (Half-)B}}                                                                                                                                                                                                     \\ \midrule
\textbf{Metrics}                & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ Acc. ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}BROD16\\ Acc. ($\uparrow$)\end{tabular}} \\ \midrule
                                & \multicolumn{3}{c}{\textit{Single dataset}}                                                                                                                                                                                                      \\ \midrule
\textbf{Vanilla}                & 75.72 $\pm$ 0.2                                                                      & 8.67 $\pm$ 1.3                                                                         & 73.57 $\pm$ 1.2                                                                     \\
\textbf{Expl. Reg.}             & 77.3 $\pm$ 0.2                                                                       & 11.23 $\pm$ 2.4                                                                        & 76.72 $\pm$ 1.1                                                                     \\
\textbf{Adv. Learning}          & 75.28 $\pm$ 0.2                                                                      & 6.92 $\pm$ 1.0                                                                         & 77.12 $\pm$ 1.2                                                                     \\ \midrule
\textbf{}                       & \multicolumn{3}{c}{\textit{FDCL A $\to$ FDCL B}}                                                                                                                                                                                                 \\ \midrule
\textbf{Van. Transfer}          & 76.33 $\pm$ 0.6                                                                      & 11.33 $\pm$ 0.7                                                                        & 70.35 $\pm$ 2.4                                                                     \\
\textbf{Expl. Reg. Transfer}    & 76.22 $\pm$ 0.5                                                                      & 7.26 $\pm$ 3.3                                                                         & 69.29 $\pm$ 1.8                                                                     \\
\textbf{Adv. Transfer}          & 75.88 $\pm$ 0.4                                                                      & 7.14 $\pm$ 3..3                                                                        & 71.11 $\pm$ 1.6                                                                     \\ \midrule
\textbf{}                       & \multicolumn{3}{c}{\textit{GHC A + FDCL A $\to$ FDCL B}}                                                                                                                                                                                         \\ \midrule
\textbf{Van. + Van.}            & 77.34 $\pm$ 0.4                                                                      & 7.79 $\pm$ 2.9                                                                         & 72.96 $\pm$ 1.5                                                                     \\
\textbf{Expl. Reg + Expl. Reg.} & 76.21 $\pm$ 0.4                                                                      & 9.00 $\pm$ 2.5                                                                         & 73.10 $\pm$ 1.4                                                                     \\
\textbf{Expl. Reg + Adv.}       & 76.94 $\pm$ 0.4                                                                      & 10.29 $\pm$ 0.4                                                                        & 76.55 $\pm$ 0.7                                                                     \\ \midrule
                                & \multicolumn{3}{c}{\textit{Stf. A + FDCL A $\to$ FDCL B}}                                                                                                                                                                                        \\ \midrule
\textbf{Van. + Van.}            & 77.18 $\pm$ 0.5                                                                      & 10.99 $\pm$ 2.8                                                                        & 71.12 $\pm$ 1.2                                                                     \\
\textbf{Expl. Reg + Expl. Reg.} & 77.13 $\pm$ 0.3                                                                      & 12.15 $\pm$ 1.2                                                                        & 72.17 $\pm$ 1.6                                                                     \\
\textbf{Expl. Reg + Adv.}       & 76.64 $\pm$ 0.6                                                                      & 6.47 $\pm$ 0.4                                                                         & 76.55 $\pm$ 0.6                                                                     \\ \bottomrule
\end{tabular}}
\caption{}

\end{table}

==> floats/legacy/tab_gab_stf_cross_domain.tex <==
% Please add the following required packages to your document preamble $\pm$ 
% \usepackage{booktabs}
\begin{table*}[]
\vspace{-0.3cm}
\centering
\scalebox{0.64}{
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
\textbf{Method / Datasets}   & \multicolumn{4}{c|}{\textbf{GHC}}                                                                                                                                                                                                                                                                                        & \multicolumn{4}{c}{\textbf{Stormfront}}                                                                                                                                                                                                                                                                                  \\ \midrule
\textbf{Metrics}             & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ F1 ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}NYT\\ Acc ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ F1 ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}NYT\\ Acc ($\uparrow$)\end{tabular}} \\ \midrule
                             & \multicolumn{4}{c|}{\textit{Single dataset}}                                                                                                                                                                                                                                                                             & \multicolumn{4}{c}{\textit{Single dataset}}                                                                                                                                                                                                                                                                                       \\ \midrule
\textbf{Vanilla}             & \textbf{49.60 $\pm$ 1.0}                                                                      & 46.43 $\pm$ 2.5                                                                        & 20.01 $\pm$ 5.7                                                                    & 72.08 $\pm$ 7.3                                                               & \textbf{53.74 $\pm$ 2.8}                                                                    & 18.09 $\pm$ 2.7                                                                        & 11.51 $\pm$ 5.1                                                                    & 73.06 $\pm$ 10                                                                \\
\textbf{Expl. Reg.}          & 43.37 $\pm$ 1.8                                                                    & \textbf{29.29 $\pm$ 1.2}                                                                        & \textbf{4.2 $\pm$ 1.6}                                                                      & \textbf{81.22 $\pm$ 11}                                                                & 51.53 $\pm$ 1.1                                                                    & \textbf{13.43 $\pm$ 1.5}                                                                        & \textbf{3.8 $\pm$ 0.4}                                                                      & \textbf{83.73 $\pm$ 8.0}                                                                 \\ 
\textbf{Emb. Zero-out}          &             43.76 $\pm$ 0.7                  &                     38.31 $\pm$ 2.0                                               &            11.95 $\pm$ 2.7                                       &                83.21 $\pm$ 5.2                        &           49.97 $\pm$   0.6             &        18.80 $\pm$ 2.0         &              8.20 $\pm$ 0.3                  &                   70.15 $\pm$ 4.4                  \\ \midrule
\textbf{}                    & \multicolumn{4}{c|}{\textit{Stf. $\to$ GHC}}                                                                                                                                                                                                                                                                             & \multicolumn{4}{c}{\textit{GHC $\to$ Stf.}}                                                                                                                                                                                                                                                                              \\ \midrule
\textbf{Van-Transfer}       & 47.83 $\pm$ 2.1                                                                    & 47.51 $\pm$ 4.6                                                                        & 18.03 $\pm$ 3.9                                                                    & 66.71 $\pm$ 11                                                            & 55.79 $\pm$ 1.3                                                                    & 17.83 $\pm$ 2.2                                                                        & 7.27 $\pm$ 1.7                                                                     & 76.98 $\pm$ 1.1                                                               \\
\textbf{Emb. Zero-out}       &                44.51 $\pm$    0.5               &        40.92 $\pm$ 4.2           &     12.91 $\pm$ 0.2                                           &     80.11 $\pm$ 1.2     &        52.98 $\pm$ 0.6         &              16.35 $\pm$ 0.9                  &           8.04 $\pm$ 2.1                             &             81.11 $\pm$ 1.9          \\
\textbf{\method$_{Reg}$} & \textbf{49.94 $\pm$ 1.0}                                                                    & \textbf{42.71 $\pm$ 3.8}                                                                        & \textbf{12.23 $\pm$ 3.3}                                                                    & \textbf{75.34 $\pm$ 4.8}                                                               & \textbf{56.43 $\pm$ 0.6}                                                                    & \textbf{18.03 $\pm$ 2.5}                                                                        & \textbf{6.86 $\pm$ 1.1}                                                                     & \textbf{81.18 $\pm$ 1.1}                                                               \\ \midrule
\textbf{}                    & \multicolumn{4}{c|}{\textit{Stf. + FDCL $\to$ GHC}}                                                                                                                                                                                                                                                                      & \multicolumn{4}{c}{\textit{GHC+ FDCL $\to$ Stf.}}                                                                                                                                                                                                                                                                        \\ \midrule
\textbf{Van-Transfer}         & 49.71 $\pm$ 0.3                                                                    & \textbf{45.84 $\pm$ 3.8}                                                                        & 12.43 $\pm$ 2.5                                                                    & \textbf{72.37 $\pm$ 7.4}                                                               & \textbf{56.78 $\pm$ 1.6}                                                                    & \textbf{14.26 $\pm$ 0.8}                                                                        & 11.04 $\pm$ 0.7                                                                    & 77.06 $\pm$ 5.1                                                               \\
\textbf{\method$_{Reg+Reg}$}    & \textbf{50.21 $\pm$ 1.4}                                                                    & 47.63 $\pm$ 0.7                                                                        & \textbf{12.29 $\pm$ 2.7}                                                                    & 68.44 $\pm$ 8.6                                                               & 53.87 $\pm$ 1.2                                                                    & 15.92 $\pm$ 1.2                                                                        & \textbf{8.4 $\pm$ 1.4}                                                                      & 83.71 $\pm$ 3.2                                                               \\
\textbf{\method$_{Reg+Adv}$}    & 49.89 $\pm$ 1.7                                                                    & 47.85 $\pm$ 1.2                                                                        & 21.25 $\pm$ 2.0                                                                    & 65.78 $\pm$ 5.7                                                              & 53.63 $\pm$ 0.7                                                                    & 15.52 $\pm$ 2.2                                                                        & 8.9 $\pm$ 1.6                                                                      & \textbf{84.87 $\pm$ 1.1}                                                               \\ \bottomrule
\end{tabular}
}
\vspace{0.2cm}
\caption{\textbf{Cross-domain and task} transfer learning of less biased models with GHC and Stormfront as target domains, where source domains are noted before arrow ($\to$). In-domain FPRD, IPTTS FPRD and NYT Accuracy (Acc.) measures prediction bias. The preferred outcomes for each metric are marked with arrows. We see \method~maintains in-domain prediction performance and overall reduces bias.}
\label{tab:cross_GHC_stf}
\vspace{-0.5cm}
\end{table*}



==> floats/legacy/tab_gab_stf_same_domain.tex <==
\begin{table*}[b]
\vspace{-0.2cm}
\centering
\scalebox{0.64}{
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
\textbf{Method / Datasets}      & \multicolumn{4}{c|}{\textbf{GHC (Half-)B}}                                                                                                                                                                                                                                                                               & \multicolumn{4}{c}{\textbf{Stormfront (Half-)B}}                                                                                                                                                                                                                                                                         \\ \midrule
\textbf{Metrics}                & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ F1 ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}NYT\\ Acc ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ F1 ($\uparrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}In-domain\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}IPTTS\\ FPRD ($\downarrow$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}NYT\\ Acc ($\uparrow$)\end{tabular}} \\ \midrule
                                & \multicolumn{4}{c|}{\textit{Single dataset}}                                                                                                                                                                                                                                                                             & \multicolumn{4}{c}{\textit{Single dataset}}                                                                                                                                                                                                                                                                              \\ \midrule
\textbf{Vanilla}                & 37.91 $\pm$ 2.5                                                                    & 36.54 $\pm$ 2.2                                                                        &             21.50 $\pm$ 2.8                                          & 68.55 $\pm$ 20                                                              & \textbf{55.56 $\pm$ 0.5}                                                                    & 20.81 $\pm$ 4.9                                                                        & 10.99 $\pm$ 5.6                                                                    & \textbf{66.28 $\pm$ 8.1}                                                               \\
\textbf{Expl. Reg.}             & \textbf{38.09 $\pm$ 2.7}                                                                    & \textbf{18.68 $\pm$ 0.3}                                                                        &                                     \textbf{4.82 $\pm$ 1.1}                                         & \textbf{84.05 $\pm$ 3.0}                                                                 & 53.05 $\pm$ 1.0                                                                    & \textbf{15.97 $\pm$ 1.1}                                                                        & \textbf{3.36 $\pm$ 3.3}                                                                     & 65.23 $\pm$ 10                                                                \\ \midrule
\textbf{}                       & \multicolumn{4}{c|}{\textit{GHC A $\to$ GHC B}}                                                                                                                                                                                                                                                                          & \multicolumn{4}{c}{\textit{Stf. A $\to$ Stf. B}}                                                                                                                                                                                                                                                                         \\ \midrule
\textbf{Van-Transfer}          & 42.41 $\pm$ 1.0                                                                      & 37.44 $\pm$ 1.5                                                                        & 17.67 $\pm$ 2.1                                                                    & 75.35 $\pm$ 4.2                                                               & 58.43 $\pm$ 1.2                                                                    & 17.96 $\pm$ 3.6                                                                        & 11.58 $\pm$ 4.8                                                                    & \textbf{74.12 $\pm$ 4.2}                                                               \\
\textbf{\method$_{Reg}$}    & \textbf{43.79 $\pm$ 1.9}                                                                    & \textbf{34.34 $\pm$ 3.1}                                                                        & \textbf{10.02 $\pm$ 1.1}                                                                    & \textbf{81.4 $\pm$ 1.4}                                                                & \textbf{58.56 $\pm$ 1.0}                                                                    & \textbf{16.42 $\pm$ 0.9}                                                                        & \textbf{7.51 $\pm$ 2.4}                                                                     & 69.45 $\pm$ 4.0                                                               \\ \midrule
\textbf{}                       & \multicolumn{4}{c|}{\textit{GHC A + FDCL A $\to$ GHC B}}                                                                                                                                                                                                                                                                 & \multicolumn{4}{c}{\textit{Stf. A + FDCL A $\to$ Stf. B}}                                                                                                                                                                                                                                                                \\ \midrule
\textbf{Van-Transfer}            & \textbf{44.30 $\pm$ 0.7}                                                                     & 41.06 $\pm$ 3.9                                                                        & 19.75 $\pm$ 6.9                                                                    & 74.60 $\pm$ 6.3                                                               & \textbf{57.58 $\pm$ 2.7}                                                                    & \textbf{13.97 $\pm$ 2.0}                                                                          & 11.33 $\pm$ 2.2                                                                    & 75.72 $\pm$ 7.5                                                               \\
\textbf{\method$_{Reg + Reg}$} & 42.96 $\pm$ 2.0                                                                    & 33.98 $\pm$ 3.0                                                                        & \textbf{9.30 $\pm$ 2.1}                                                                      & \textbf{86.05 $\pm$ 1.9}                                                               & 56.72 $\pm$ 1.7                                                                    & 17.91 $\pm$ 1.0                                                                        & \textbf{8.05 $\pm$ 0.6}                                                                     & \textbf{77.40 $\pm$ 0.3}                                                                \\
\textbf{\method$_{Reg + Adv}$}       & 42.44 $\pm$ 3.5                                                                    & \textbf{33.96 $\pm$ 1.5}                                                                        & 16.58 $\pm$ 1.7                                                                    & 81.79 $\pm$ 9.0                                                                 & 55.63 $\pm$ 2.5                                                                    & 17.14 $\pm$ 0.5                                                                        & 13.78 $\pm$ 4.3                                                                    & 70.37 $\pm$ 10                                                              \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Same-domain} transfer with the second half of GHC and Stormfront as the target domain.}
\label{tab:same_GHC_stf}
\end{table*}

==> floats/tab_non_transfer.tex <==
% results included for completeness

\begin{table}[]
\centering
\scalebox{0.53}{
\begin{tabular}{@{}l|cc|cc@{}}
\toprule
\textbf{Metrics}          & \textbf{In-domain F1 ($\uparrow$)} & \textbf{BROD Acc. ($\uparrow$)} & \textbf{In-domain F1 ($\uparrow$)} & \textbf{TPRD ($\downarrow$)} \\ \midrule
\textbf{Dataset} & \multicolumn{2}{c|}{\textbf{FDCL}}                                   & \multicolumn{2}{c}{\textbf{BiasBios}}                             \\ \midrule
\textbf{Vanilla}          &     &                     &  82.21 $\pm$ 0.0              &                12.01 $\pm$ 0.3                                          \\
\textbf{Expl. Reg.}       &                                    &                                 & 86.02 $\pm$ 0.3 & 12.97 $\pm$ 0.4                                         \\
\textbf{Adv. Learning}    &                                    &                                 & 85.75 $\pm$ 0.3 & 8.4 $\pm$ 0.4                                        \\ \bottomrule
\end{tabular}
}
\caption{Non-Transfer bias mitigation on FDCL and BiasBios for completeness of results.}
\end{table}
